Impact of Heavy Quark Masses on Parton Distributions and LHC Phenomenology

We present a determination of the parton distributions of the nucleon from a global set of hard scattering data using the NNPDF methodology including heavy quark mass effects: NNPDF2.1. In comparison to the previous NNPDF2.0 parton determination, the dataset is enlarged to include deep--inelastic charm structure function data. We implement the FONLL-A general-mass scheme in the FastKernel framework and assess its accuracy by comparison to the Les Houches heavy quark benchmarks. We discuss the impact on parton distributions of the treatment of the heavy quark masses, and we provide a determination of the uncertainty in the parton distributions due to uncertainty in the masses. We assess the impact of these uncertainties on LHC observables by providing parton sets with different values of the charm and bottom quark masses. Finally, we construct and discuss parton sets with a fixed number of flavours.

==> sec-f2cdata.tex <==
\section{Systematic uncertainties in HERA $F_2^c$ data}
\label{sec:appf2cdata}

We assume the same correlations between systematic uncertainties
as in the upcoming combined HERA-I $F_2^c$ dataset.

For H1 the measurements can be divided in $D^{*\pm}$ production
cross sections and inclusive track measurements. For $D^{*\pm}$
production, the following bin-to-bin correlated uncertainties 
are considered: electron energy and polar angle, 
hadronic energy, luminosity, trigger efficiency, branching ratio for 
the decay channel $D^*\to KK\pi$, 
photoproduction background, 
stability of  efficiency
due to the usage of MC simulations. 
Uncorrelated uncertainties are the extraction of the $D^{*\pm}$ 
signal, stability of the effciencies due to the variation 
of the PDF in the MC, variation of the cut on the $D^0$ mass, 
contribution of reglections to the D* signal, radiative corrections.
Partially (50\%) correlated uncertainties are 
tracking efficiency and reconstruction of the primary vertex.

On the other hand, for the vertex detector (CST) measurements we
can identify various sources of systematic uncertainties: 
impact parameter smearing, H1 drift chamber track finding efficiency, 
CST track finding efficiency, D and B  multiplicities, 
c- and b-fragmentation, QCD model uncertainty, hadronic 
energy, normalization uncertainty

==> sec-massive-cc.tex <==
\section{Mellin space results -- charged current scattering}
\label{sec:massive-cc}

In this section we compute the analytical Mellin transforms of the
massive heavy quark coefficient functions in charged current
deep--inelastic scattering. The $\mathcal{O}\lp \alpha_s\rp$
expressions were computed in Refs.. .

The charm structure functions in CC scattering in the
massive scheme read
\begin{multline}
\mathcal{F}_{i,h}^{(n_l)}(x,Q^2)=
s'(\xi,\mu^2)+
\frac{\alpha_s(\mu^2)}{2\pi}
\bigg\{\int\limits_{\xi}^{1}\frac{d\xi'}{\xi'}\bigg[C^{(n_l)}_{i,h}(\xi',\mu^2,\lambda)s'(\frac{\xi}{\xi'},\mu^2)+\\
+C^{(n_l)}_{i,g}(\xi',\mu^2,\lambda)g(\frac{\xi}{\xi'},\mu^2)
\bigg]\bigg\}=\\=s'(x,\mu^2)+
\frac{\alpha_s(\mu^2)}{2\pi}
\bigg\{\int\limits_{x}^{1}\frac{dx'}{x'}\theta(W^2-m_c^2)\bigg[C^{(n_l)}_{i,h}(x',\mu^2,\lambda)s'(\frac{x}{x'},\mu^2)+\\
+C^{(n_l)}_{i,g}(x',\mu^2,\lambda)g(\frac{x}{x'},\mu^2)
\bigg]\bigg\}
\label{eq:ccsf}
\end{multline}
with $$s'\equiv |V_{cs}|^2s+|V_{cd}|^2\frac{d+u}{2}$$
 $$\xi=x(1+\frac{m_c^2}{Q^2})$$
 and $\mathcal{F}_1^c\equiv F_{1,h}^{(n_l)}$,\,$\mathcal{F}_2^c\equiv\frac{F_2^c}{2\xi}$,\,$\mathcal{F}_3^c\equiv\frac{F_3^c}{2}$. 

For a generic structure function,
\be
F(x,Q^2,\lambda)=\int_{x/\lambda}^1 \frac{dy}{y}C^{(n_l)}\lp y,\lambda,\as\rp
q\lp \frac{x}{\lambda y},Q^2\rp
\ee
it can be shown that its Mellin transform 
\be
F(N,Q^2,\lambda)= C^{(n_l)}\lp N,\lambda,\as\rp
q\lp N,Q^2\rp
\ee
is given in terms of Mellin moments of the $x-$space
coefficient functions in Eq.\ref{eq:ccsf}
\be
 C^{(n_l)}\lp N,\lambda,\as\rp = \int_0^\lambda dz z^{N-1}
C^{(n_l)}\lp z/\lambda,\lambda,\as\rp =
\lambda^N\int_0^1 dz z^{N-1}
C^{(n_l)}\lp z,\lambda,\as\rp \ .
\ee

The $x-$space explicit expressions at $\mathcal{O}\lp \alpha_s\rp$
of the CC massive coefficient functions  given in Ref. can
be transformed to $N-$space, yielding

and for gluons
The Mellin transforms of the massive CC HQ gluon coefficients
are straightforward: the various coefficient functions
read:
\begin{eqnarray}
C_{1,g}^{(n_l)}&=&\frac{1}{2}[z^2+(1-z)^2]\bigg(\ln\frac{1-\lambda z}{(1-\lambda)z}+2\ln(1-z)-\ln(1-\lambda z)-\ln z\bigg)+\nonumber\\
&+&[4-4(1-\lambda)]z(1-z)+\frac{(1-\lambda)z}{1-\lambda z}-1+(1-\lambda)z\ln\frac{1-\lambda z}{(1-\lambda)z}(2-4\lambda z)\nonumber
\end{eqnarray}
\begin{eqnarray}
C_{2,g}^{(n_l)}&=&\frac{1}{2}[z^2+(1-z)^2]\bigg(\ln\frac{1-\lambda z}{(1-\lambda)z}+2\ln(1-z)-\ln(1-\lambda z)-\ln z\bigg)+\nonumber\\
&+&[8-18(1-\lambda)+12(1-\lambda)^2]z(1-z)+\frac{1-\lambda}{1-\lambda z}-1+(1-\lambda)z\ln\frac{1-\lambda z}{(1-\lambda)z}(6\lambda-12\lambda^2 z)\nonumber
\end{eqnarray}
\begin{eqnarray}
C_{3,g}^{(n_l)}&=&\frac{1}{2}[z^2+(1-z)^2]\bigg(\ln\frac{1-\lambda z}{(1-\lambda)z}+2\ln(1-z)-\ln(1-\lambda z)-\ln z\bigg)+\nonumber\\
&+&2(1-\lambda)z(1-z)+(1-\lambda)z\ln\frac{1-\lambda z}{(1-\lambda)z}[2z(1+\lambda )-2]
\end{eqnarray}

The massless limit of the $x-$space coefficient functions read
for gluons
\begin{eqnarray}
C_{2,g}^{(n_l,0)}&=&[z^2+(1-z)^2]\bigg(\ln \frac{1-z}{z}+\frac{1}{2}\ln\frac{Q^2+m^2}{m^2} \bigg) + \lp 8z(1-z)-1\rp
\end{eqnarray}
and for quarks
which in N-space yield

The final expression of the Mellin space heavy quark coefficient
functions for CC DIS read

\subsubsection*{Quark Initiated Processes}
\begin{multline}
%
C^{(n_l)}_{1,q}(N,Q^2)=\frac{4}{3}\bigg\{
%A8
-\Big(\frac1N - \frac1{N+1} - 2 S_1\Big)\ln\lambda
%1
-\bigg(4+\frac{1}{2\lambda}+
\frac{\pi^2}{3}+\frac{1+3\lambda}{2\lambda}K_A\bigg)+
\\\\
%A1
-2(S_2-\zeta_2)+\frac{1}{N^2}-\frac{1}{(N+1)^2}+
\\\\
%A2
+\frac13\bigg[\frac3{N^2}+\frac{3}{(N+1)^2}+6\gamma\left(\gamma+\frac1N+\frac1{N+1}\right) + \pi^2+3\left(S_1-\frac1N-\gamma\right)\left(3\gamma+S_1-\frac1N\right)+
\\\\
+3\left(S_1 + \frac{1}{N+1}-\gamma\right)^2-6\left(\zeta_2-S_2+\frac{1}{N^2}\right)\bigg]+
\\\\
%A3
+J_{\lambda}(N)
%A4
+ \frac{1}{N}-\frac{1}{N+1}+ 2S_1+
\\\\
%A5
%+(z-z^2)\frac{1}{(1-\lambda z)_+}
+\frac{_2F_1(1,N+1,N+2;\lambda)}{N+1}-\frac{_2F_1(1,N+2,N+3;\lambda)}{N+2}
%A6
%+\frac{1}{2}\bigg[\frac{1-z}{(1-\lambda z)^2}\bigg]_+
+\frac{1}{2}\frac{ _2F_1(2,N,N+2;\lambda)}{N(N+1)}
%
\bigg\}
\end{multline}
where
\begin{equation}
J_{\lambda}(N) = \sum_{k=1}^{\infty}\frac{2\lambda^k}{k}\left[S_1(N+k)-S_1(k)-\frac1{2(N+k)(N+k+1)}\right]
\end{equation}


% \begin{multline}
% J_{\lambda}(N)=\sum_{\alpha=1}^\infty\bigg[\frac{\lambda^\alpha}{\alpha}\Big(\psi(\alpha+1)+\psi(\alpha+3)-\psi(N+\alpha)-\psi(N+2+\alpha)\Big)\bigg]
% \end{multline}
\begin{multline}
%inizio primo termine
C^{(n_l)}_{2,q}(N,Q^2)=\frac{4}{3}\bigg\{
%A8
-\Big(\frac1N - \frac1{N+1} - 2 S_1\Big)\ln\lambda
%1
-\bigg(4+\frac{1}{2\lambda}+
\frac{\pi^2}{3}+\frac{1+3\lambda}{2\lambda}K_A\bigg)+
\\\\
%A1
-2(S_2-\zeta_2)+\frac{1}{N^2}-\frac{1}{(N+1)^2}+
\\\\
%A2
+\frac13\bigg[\frac3{N^2}+\frac{3}{(N+1)^2}+6\gamma\left(\gamma+\frac1N+\frac1{N+1}\right) + \pi^2+3\left(S_1-\frac1N-\gamma\right)\left(3\gamma+S_1-\frac1N\right)+
\\\\
+3\left(S_1 + \frac{1}{N+1}-\gamma\right)^2-6\left(\zeta_2-S_2+\frac{1}{N^2}\right)\bigg]+
\\\\
%A3
+J_{\lambda}(N)
%1
+ K_A+
%A7
2\frac{_2F_1(1,N-1,N;\lambda)}{N-1}-\frac{_2F_1(1,N,N+1;\lambda)}{N}-\frac{_2F_1(1,N+1,N+2,\lambda)}{N+1}+
\\\\
+2\left(S_1 + \frac{1}{N+1} - \frac{1}{N-1}\right)
%A6
%+\frac{1}{2}\bigg[\frac{1-z}{(1-\lambda z)^2}\bigg]_+
+\frac{1}{2}\frac{ _2F_1(2,N,N+2;\lambda)}{N(N+1)}
%
\bigg\}
\end{multline}
\begin{multline}
%inizio primo termine
C^{(n_l)}_{3,q}(N,Q^2)=\frac{4}{3}\bigg\{
%A8
-\Big(\frac1N - \frac1{N+1} - 2 S_1\Big)\ln\lambda
%1
-\bigg(4+\frac{1}{2\lambda}+
\frac{\pi^2}{3}+\frac{1+3\lambda}{2\lambda}K_A\bigg)+
\\\\
%A1
-2(S_2-\zeta_2)+\frac{1}{N^2}-\frac{1}{(N+1)^2}+
\\\\
%A2
+\frac13\bigg[\frac3{N^2}+\frac{3}{(N+1)^2}+6\gamma\left(\gamma+\frac1N+\frac1{N+1}\right) + \pi^2+3\left(S_1-\frac1N-\gamma\right)\left(3\gamma+S_1-\frac1N\right)+
\\\\
+3\left(S_1 + \frac{1}{N+1}-\gamma\right)^2-6\left(\zeta_2-S_2+\frac{1}{N^2}\right)\bigg]
%A3
+J_{\lambda}(N)
%A8
+\frac1N - \frac1{N+1} - 2 S_1+
\\\\
%A9
+\frac{_2F_1(1,N,N+1;\lambda)}{N}-\frac{_2F_1(1,N+1,N+2;\lambda)}{N+1}
%A6
%+\frac{1}{2}\bigg[\frac{1-z}{(1-\lambda z)^2}\bigg]_+
+\frac{1}{2}\frac{ _2F_1(2,N,N+2;\lambda)}{N(N+1)}
%qui
\bigg\}
\end{multline}


\subsubsection*{Gluon Initiated Processes}
\begin{multline}
%primo termine 
C^{(n_l)}_{1,g}(N,Q^2)=-\frac12\left[\frac2{N+2}-\frac{2}{N+1}+\frac1N\right]\ln\lambda+\\\\+   \frac{4-2(N-3)N-N(N^2+N+2)(\ln(1-\lambda)+2S_1)}{2N^2(N+1)(N+2)}+\\\\
+\Big(4-4(1-\lambda)\Big)\bigg(\frac{1}{N+1}-\frac{1}{N+2}\bigg)+(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)}{N+1}-\frac{1}{N}+\\\\
+2(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)}{(N+1)^2}-4(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)-1}{(N^2+3N+2)}
\end{multline}
\begin{multline}
C^{(n_l)}_{2,g}(N,Q^2)=-\frac12\left[\frac2{N+2}-\frac{2}{N+1}+\frac1N\right]\ln\lambda+ \\\\+\frac{4-2(N-3)N-N(N^2+N+2)(\ln(1-\lambda)+2S_1)}{2N^2(N+1)(N+2)}+\\\\
+\frac{2-6\lambda+12\lambda^2}{N^2+3N+2}+(1-\lambda)\frac{\;_2F_1(1,N,N+1,\lambda)}{N}-\frac{1}{N}+\\\\
+6\lambda(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)}{(N+1)^2}-12\lambda(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)-1}{(N^2+3N+2)}
\end{multline}
\begin{multline}
C^{(n_l)}_{3,g}(N,Q^2)=-\frac12\left[\frac2{N+2}-\frac{2}{N+1}+\frac1N\right]\ln\lambda+ \\\\+\frac{4-2(N-3)N-N(N^2+N+2)(\ln(1-\lambda)+2S_1)}{2N^2(N+1)(N+2)}+
2(1-\lambda)\bigg(\frac{1}{N+1}-\frac{1}{N+2}\bigg)+\\\\
-2(1-\lambda)\frac{\;_2F_1(1, N+1, N+2, \lambda)}{(N+1)^2}+2(1-\lambda^2)\frac{\;_2F_1(1, N+1, N+2, \lambda)-1}{\lambda(N^2+3N+2)}
\end{multline}


==> sec-pdfevol.tex <==
%-----------------------------------------------------------------------------------------------------------

\section{Heavy Quark effects in FastKernel}
\label{sec:evolution}

The major improvement in the FastKernel framework as compared
to Ref.\cite{Ball:2010de} 
is the inclusion of heavy quark mass effects in deep--inelastic
scattering structure functions. Heavy quarks are included following
the FONLL general-mass scheme\cite{Forte:2010ta}. In particular we will use the
FONLL-A scheme with threshold damping factor. In this section
we describe the details of the implementation of FONLL in FastKernel,
and compute the LH HQ benchmark tables to show the accuracy of the
implementation.

\subsection{Implementation of the FONLL scheme in FastKernel}
In this section we review the FONLL General Mass scheme,
presented in \cite{Forte:2010ta}, and describe its implementation in the
FastKernel framework.

The FONLL-A GM scheme prediction for
the a generic charm structure function can be written in $N--$space
as follows:
\bea
\label{eq:f2c_nnpdf}
F_{c}^{\rm FONLL}(N,Q^2) &=& 
F_{c}^{(n_l)}(N,Q^2) \\
&-&\theta\lp Q^2 - m^2\rp\lp 1-\frac{m^2}{Q^2}\rp^2 \lc
F_{c}^{(n_l,0)}(N,Q^2)-F_{h}^{(n_l+1)}(N,Q^2) \rc \nonumber
\eea
The explicit expressions of the analytic Mellin transforms
of the massive NC and CC heavy quark coefficient functions
(and their associated massless limits)
are given in the appendices \ref{sec:massive-nc} and
\ref{sec:massive-cc}.

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.99\textwidth]{plots/f2c-schemes.eps}
\includegraphics[width=0.99\textwidth]{plots/flc-schemes.eps}
\end{center}
\caption{\small The charm structure functions $F_2^c(x,Q^2)$ 
and $F_L^c(x,Q^2)$ 
as a function of $Q^2$ for different values of $x$ from
$x=10^{-5}$ to $x=10^{-2}$ in various 
heavy quark schemes, computed using the FastKernel method:
FONLL-A-Damp, ZM-VFN and the FFN scheme. The iterated
solution of the DGLAP evolution equations has been used, and the
PDFs and settings are identical to those of the Les Houches
Heavy quark benchmark comparison.}
\label{fig:f2c_vs_q2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.49\textwidth]{plots/f2c-schme-diff.eps}
\includegraphics[width=0.49\textwidth]{plots/f2p-schme-diff.eps}
\includegraphics[width=0.49\textwidth]{plots/flc-schme-diff.eps}
\includegraphics[width=0.49\textwidth]{plots/flp-schme-diff.eps}
\end{center}
\caption{\small The relative
difference for the charm structure functions $F_2^c(x,Q^2)$ 
and $F_L^c(x,Q^2)$ computed in the ZM and in the GM schemes
(FONLL-A-Damp)
as a function of $x$ and $Q^2$. The
PDFs and settings are identical to those of the Les Houches
Heavy quark benchmark comparison.}
\label{fig:f2c_flc_cont}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

As an illustration of the differences between various HQ schemes,
in Fig.\ref{fig:f2c_vs_q2} we compare the $F_2^c$ structure
function for various heavy quark schemes: ZM, FONLL-A-Damp
and the FFN scheme as a function of $Q^2$ for different values of
$x$. It can easily be seen how FONLL-A-Damp smoothly interpolates
between the FFN scheme near threshold and the massless scheme
at large $Q^2$. This smooth matching is guaranteed by the 
damping factor in Eq. which acts as a threshold suppression factor,
in analogy with $\chi--$scaling in S-ACOT-$\chi$. Note that 
the PDFs and settings are identical to those of the Les Houches
Heavy quark benchmark comparison.

The impact of heavy quark effects in DIS structure
functions is further quantified in Fig.\ref{fig:f2c_flc_cont},
where the relative difference between the ZM and FONLL-A-Damp
schemes is computed as a function of $x$ and $Q^2$, both
for the inclusive structure functions $F_2^p$ and $F_L^p$ and
for the charm structure functions $F_2^c$ and $F_L^c$. For the
phenomenologically more relevant case of $F_2^p$, we see that
heavy quark mass effects can be as large as $\sim 10\%$, decreasing
fast for increasing $x$ and $Q^2$. As in the case of Fig.\ref{fig:f2c_vs_q2} 
the Les Houches heavy quark benchmark settings have been used.

\subsection{Heavy Quark Benchmarking}


As a check that the implementation of the FONLL General-Mass scheme
into the FastKernel framework has the required accuracy, in 
Table\ref{tab:tablebench} for $F_2^c$ and in Table
\ref{tab:tablebench2} for $F_L^c$,
we compare the results for the Les Houches Heavy Quark benchmarks
for FONLL-A-Damp obtained with the FONLLdis code\cite{Forte:2010ta} 
and with the
FastKernel framework for various relevant values of $Q^2$. The
benchmark settings for the PDFs and $\alpha_s$ are used for
this comparison. What we can see is that the accuracy on
$F_2^c$ is essentially always below the percent level, enough
for precision phenomenological studies.


%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\begin{center}
\scriptsize
 \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{3}{|c|}{FONLL-A-Damp} & \multicolumn{3}{|c|}{FFN} \\
 \hline
 $x$ & FONLLdis & FastKernel  
& Accuracy & FONLLdis & FastKernel  
& Accuracy\\
\hline
 \hline
\multicolumn{7}{|c|}{$Q^2=4$ GeV$^2$} \\
 \hline
$10^{-5}$ &      0.1507  & 0.1501   & $0.4\%$  & 0.1088& 0.1091& $0.3\%$\\
 $10^{-4}$  &    0.0936  & 0.0931   & $0.5\%$  & 0.0697& 0.0698& $0.1\%$ \\
 $10^{-3}$  &    0.0506   & 0.0504  & $0.4\%$  & 0.0392& 0.391&$0.2\%$ \\
  $10^{-2}$  &   0.0174   & 0.0177 & $1.5\%$  & 0.0136& 0.0137& $0.7\%$\\
\hline
\hline
\multicolumn{7}{|c|}{$Q^2=10$ GeV$^2$} \\
 \hline
$10^{-5}$ &    0.563 & 0.561 & $0.4\%$  & 0.3598 & 0.3602& $0.1\%$\\
 $10^{-4}$  &  0.312 & 0.311 & $0.3\%$  & 0.2007&0.2011& $0.2\%$\\
 $10^{-3}$  &   0.1499 & 0.1495 & $0.3\%$  & 0.0981& 0.0982& $0.1\%$\\
  $10^{-2}$  &  0.05056 & 0.05052 & $0.1\%$  & 0.0328 & 0.0327& $0.3\%$ \\
\hline
\hline
\multicolumn{7}{|c|}{$Q^2=100$ GeV$^2$} \\
 \hline
$10^{-5}$ &    2.28636 & 2.28577 & $0.02\%$  & 1.9779 & 1.9877& $0.5\%$ \\
 $10^{-4}$  &  1.12186 & 1.12082 & $0.1\%$  & 0.9161& 0.9184& $0.3\%$\\
 $10^{-3}$  &  0.48008 & 0.47919 & $0.2\%$  & 0.3644& 0.3647& $0.1\%$\\
  $10^{-2}$  & 0.15207 & 0.15200 & $0.04\%$  & 0.1037 & 0.1038& $0.1\%$\\
 \hline
 \end{tabular}
\end{center}
\caption{\small Results of the benchmark comparison for the
$F_{2c}(x,Q^2)$ structure function in the
 FONLL-A-Damp scheme for the FONLLdis code\cite{Forte:2010ta}
and for the FastKernel framework. Results are provided at the
benchmark kinematical points in $x,Q^2$. For completeness
we also show the analogous results for the case of
the massive scheme results.
\label{tab:tablebench}}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\begin{center}
\scriptsize
 \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
& \multicolumn{3}{|c|}{FONLL-A-Damp} & \multicolumn{3}{|c|}{FFN} \\
 \hline
 $x$ & FONLLdis & FastKernel  
& Accuracy & FONLLdis & FastKernel  
& Accuracy\\
\hline
 \hline
\multicolumn{7}{|c|}{$Q^2=4$ GeV$^2$} \\
 \hline
$10^{-5}$ &    0.0130174  & 0.013094  & $0.6\%$ & 0.009077 & 0.009081 & \\
 $10^{-4}$  &  0.008347  & 0.008316 & $0.4\%$ & 0.005913 & 0.005910 & \\
 $10^{-3}$  &  0.004795  & 0.004778 & $0.3\%$ & 0.003511 & 0.003509 & \\
  $10^{-2}$  & 0.001910  & 0.001907 & $0.2\%$  & 0.001403 & 0.001406 & \\
\hline
\hline
\multicolumn{7}{|c|}{$Q^2=10$ GeV$^2$} \\
 \hline
$10^{-5}$ & 0.073235   & 0.073022   & $0.3\%$ & 0.049856 & 0.049982& \\
 $10^{-4}$  & 0.041392 &  0.041251 & $0.3\%$ & 0.028402 & 0.028423 & \\
 $10^{-3}$  & 0.020754  & 0.020707 & $0.2\%$ & 0.014463 & 0.014456 & \\
  $10^{-2}$  & 0.007616  & 0.007595  & $0.3\%$ & 0.005350 & 0.005346 & \\
\hline
\hline
\multicolumn{7}{|c|}{$Q^2=100$ GeV$^2$} \\
 \hline
$10^{-5}$ & 0.471889   & 0.4729 & $0.2\%$ & 0.3955& 0.397855 & \\
 $10^{-4}$  & 0.2236  & 0.2235 & $0.1\%$ & 0.18656 & 0.186914 & \\
 $10^{-3}$  &  0.0920 & 0.09188 & $0.1\%$ & 0.0765 & 0.076393 & \\
  $10^{-2}$  & 0.027822  &  0.02782 & $0.1\%$& 0.023079 & 0.023100 & \\
 \hline
 \end{tabular}
\end{center}
\caption{\small Same as Table \ref{tab:tablebench} for the
$F_{Lc}(x,Q^2)$ structure function.
\label{tab:tablebench2} 
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%

As an alternative to the use of a General Mass scheme in PDF analysis,
some groups have advocated the use of the Fixed Flavor Number scheme,
in which the charm and bottom quarks are always treated as massive
partons regardless of the value of $Q^2$. In the FFN large
logarithms of the type $\ln^k Q^2/m_h^2$ are not resummed into
the heavy quark PDFs, as done in the GM schemes. In order to quantify
the differences between the GM and FFN schemes, we will perform
as well a version of the NNPDF2.1 fit using the $N_f=3$ FFN scheme.
The differences with respect the GM scheme are essentially two:
the use of the FFN coefficient functions instead of the FONLL
ones, and the use of a $N_f=3$ running $\alpha_s(Q^2)$. For consistency
with the GM analysis, instead of the GM default
$\alpha_s\lp M_Z\rp_{N_f=5}=0.119$ we will 
take $\alpha_s\lp M_Z\rp_{N_f=3}=0.1056$,
which follows from the equality
\be
\alpha_s\lp m_c\rp_{N_f=3}=\alpha_s\lp m_c\rp_{N_f=3}
\ee


Now we discuss the benchmarking of the heavy quark implementation in
the charged current sector. 

{\bf discussion CC}

Now we turn the discussion to the charged current structure functions.
{\bf table with numbers for dimuons, compare ZM, I-ZM, S-ACOT, FONLL}.

Note that the fact that, as suggested in Ref.\cite{Nadolsky:2009ge} 
the Improved Zero Mass
scheme for dimuons leads to results which are very close numerically
to the FFN scheme implies that all results related to strangeness
determination will be robust also after the proper treatment of
mass effects in the charged current section.

%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\begin{center}
\includegraphics[width=0.99\textwidth]{plots/ccbench.eps}
\end{center}
\caption{\small The charm production cross section
in CC scattering in the kinematics of the NuteV
dimuon data.
Several
heavy quark schemes are compared, computed using the FastKernel method:
FONLL-A-Damp (which coincides with the FFN
scheme in this case), ZM-VFN, I-ZM-ZM scheme. The
PDFs and settings are identical to those of the Les Houches
Heavy quark benchmark comparison. We also compare with the
benchmark computation corresponding to the S-ACOT-$\chi$ general
mass scheme. {\bf All data bins, add FFN scheme with FastKernel}} 
\label{fig:f2c_vs_q2}
\end{figure}
%%%%%%%%%%%%%%%%%%%%

==> tab-chi2.tex <==
\begin{table}
\centering
\small
\begin{tabular}{|c|c|c|c|c|}
\hline
Experiment & Set     &   NNPDF2.0  & NNPDF2.0 + FONLL-A &  NNPDF2.1  \\
\hline
\hline
 NMC-pd  &         &    1.04  & 1.03 &  0.96  \\
NMC     &        &    1.69  & 1.51 & 1.61 \\
SLAC & & & 1.31 & 1.31 \\
& SLACp         &    1.57   & 1.48  & 1.41  \\
& SLACd            &         1.14 & 1.14 &  1.13  \\
BCDMS & & & 1.19 & 1.21\\
& BCDMSp          &   1.30  & 1.18 &1.22 \\
& BCDMSd          &  1.16   & 1.13 & 1.11  \\
HERA1-av & & & 1.28 & 1.11\\
&HERA1-NCep    & 1.32  & 1.56  &  1.29  \\
&HERA1-NCem     & 0.85  & 0.88 &  0.82  \\
&HERA1-CCep     &    0.97 & 0.97 &   0.96  \\
&HERA1-CCem     &   0.57  & 0.57&  0.57 \\
CHORUS & &1.18 & 1.18 & 1.19 \\
&CHORUSnu       & 1.26  & 1.26&  1.26  \\
&CHORUSnb   &   1.04  &  1.04 & 1.05  \\
FLH108       &  &   1.50  & 1.29  & 1.32  \\
NTVDMN & & 0.71 & 0.71 & 0.71 \\
&NTVnuDMN      &  0.72  & 0.72 & 0.54  \\
&NTVnbDMN       &  0.70  & 0.70 & 0.81  \\
ZEUS-H2 & & & 1.27 & 1.23 \\
&Z06NC          &   1.17   &  1.19& 1.14 \\
&Z06CC           &  1.27   & 1.27 &1.25 \\
ZEUSF2C & & 1.80 &  2.14 & 1.89 \\
& ZEUSF2C99      & {\it 1.99} & {\it 1.81}& 1.57\\
& ZEUSF2C03      & {\it 2.54}& {\it 3.64}& 3.22 \\
& ZEUSF2C08      & {\it 0.71}& {\it 0.38}& 0.34 \\
& ZEUSF2C09      & {\it 0.28}& {\it 0.11}& 0.11\\
H1F2C & &  1.67 & 1.70 &  1.59\\
& H1F2C04        & {\it 1.29}& {\it 1.09} & 1.07 \\
& H1F2C05        & {\it 2.98}& {\it 1.79}& 1.62 \\
& H1F2C09        & {\it 3.01}& {\it 2.62}&  2.57\\
& H1F2C10    & {\it 1.26}& {\it 1.45} & 1.34\\
DYE605   & & 0.85  & 0.85 & 0.82 \\
DYE866 & &1.24 & 1.24 & 1.32\\
& DYE866p       &   1.27&  1.27 &  1.32 \\
& DYE866r        &  0.87& 0.87 &  0.70  \\
CDFWASY     &   &   1.84 & 1.84 & 2.10  \\
CDFZRAP     &   &    1.98& 1.98 &   1.83 \\
D0ZRAP      &  &   0.56  & 0.56 & 0.56   \\
CDFR2KT      &   &    0.79 & 0.79 &  0.79 \\
D0R2CON      &  &   0.92  & 0.92 & 0.91  \\
\hline
\end{tabular}
\caption{\small Table of $\chi^2$ of the various experiments included
in the NNPDF2.1 fit compared to the NNPDF2.0 fit. The NNPDF2.0 + FONLL-A
columns indicate which is the results for the $\chi^2$ when the NNPDF2.0
PDFs are combined with the FONLL-A-Damp coefficient functions. Experiments
which are not included in the fit (the $F_2^c$ HERA data) are marked
with black font. Note that we show both the $\chi^2$ of experiments
and sets (see Ref. for the distiction between these) in the
case in which one experiments corresponds to more than one set, so in the
latter case cross correlations between sets of the same experiment are
neglected. Note that all the $\chi^2$ have been obtained with
the corresponding NNPDF sets of 1000 replicas. Note also that for hadronic
data the first two columns are identical since the ZM-VFN scheme is
used in both cases. \label{tab:chi2}}
\end{table}

==> tab-exps-sets.tex <==
 \begin{table}
 \scriptsize
 \centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|}
  \hline
  Experiment & Set & Ref. & Points & $x_{\rm min}$ & $x_{\rm max}$
 & $Q^2_{\rm min}$ & $Q^2_{\rm max}$  \\ \hline
\hline
 ZEUSF2C         & &    &       69 (62) & & & & \\ \hline
 &  ZEUSF2C99       & \cite{Breitweg:1999ad} &  21 (18) &      $5\,10^{-5}$ 
($1.3\,10^{-4}$) &      0.02 &        1.8 (4) &      130 \\
 \hline
 &  ZEUSF2C03       &  \cite{Chekanov:2003rb}& 31 (27) &      $3\,10^{-5}$ 
($7\,10^{-5}$)&      0.03 &        2.0 (4.0) &      500\\
 \hline
 &  ZEUSF2C08       & \cite{Chekanov:2008yd}  & 9 &      $2.2\,10^{-4}$ &      0.032 &        7.0 &      112  \\
 \hline
 &  ZEUSF2C09       &  \cite{Chekanov:2009kj} & 8 &      $8\,10^{-4}$ &      0.03 &       30 &     1000 \\
 \hline
\hline
 H1F2C           &  &     &      47 (45)  & & & & \\ 
 \hline
&  H1F2C01         & \cite{Adloff:2001zj} & 12 (10) &      $5\,10^{-4}$ &      $3.2\,10^{-3}$ &        1.5 &       60   \\
\hline
 &  H1F2C09         & \cite{Collaboration:2009jy}  & 6 &      $2.4\,10^{-4}$ &      0.025 &      120 &      400  \\
\hline
 &  H1F2C10         & \cite{H1F2c10:2009ut}   &29 &      $2\,10^{-4}$ &      0.05 &        5.0 &     2000  \\
 \hline
\hline
Total &        &    &3554 &     &&&\\
 \hline
 \end{tabular}
\caption{\label{tab:exps-sets} \small Kinematical coverage
 of the various $F_2^c(x,Q^2)$ HERA
data sets included in the present analysis. In parenthesis results
after kinematical cuts. The last line gives the total number of
datapoints included in the NNPDF2.1 analysis.}
 \end{table}


 \begin{table}
 \scriptsize
 \centering
 \begin{tabular}{|c|c|c|c|c|c|c|}
  \hline
  Experiment & Set & Ref. & $\sigma_{\rm stat}$ (\%)& 
    $\sigma_{\rm sys}$ &  $\sigma_{\rm norm}$(\%)&  $\sigma_{\rm tot}$ (\%) \\ \hline
\hline
 ZEUSF2C         & &    &       69 (62) & & &\\ \hline
 &  ZEUSF2C99       & \cite{Breitweg:1999ad} &   15.9 &  14.0 &   1.6 &  21.4 \\
 \hline
 &  ZEUSF2C03       &  \cite{Chekanov:2003rb}&   11.2 &  14.8 &   2.2 &  19.0 \\
 \hline
 &  ZEUSF2C08       & \cite{Chekanov:2008yd}  & 15.5 &  27.0 &   2.6 &  31.4 \\
 \hline
 &  ZEUSF2C09       &  \cite{Chekanov:2009kj} & 15.9 &  23.3 &   2.6 &  28.5 \\
 \hline
\hline
 H1F2C           &  &     &      47 (45)  & & &  \\ 
 \hline
&  H1F2C01         & \cite{Adloff:2001zj} &  26.4 &   0.0 &   1.5 &  26.4 \\
\hline
 &  H1F2C09         & \cite{Collaboration:2009jy}  19.0 &   9.9 &   2.6 &  21.6 \\
 \hline
 &  H1F2C10         & \cite{H1F2c10:2009ut}   &  8.0 &  12.0 &   2.6 &  14.9 \\
 \hline
 \end{tabular}
\caption{\label{tab:exps-sets-err} \small Average of the various
experimental uncertainties of the $F_2^c(x,Q^2)$ HERA
data sets included in the present analysis.}
 \end{table}


